Practical Limits to Single-Mode Vacuum Squeezing with a SNAIL Parametric Amplifier

We characterize single-mode vacuum squeezing generated by a SNAIL Parametric Amplifier (SPA) operated under conditions representative of practical sensing and qubit-readout experiments. Motivated by prior expectations that Kerr-induced distortion limits squeezing in degenerate parametric amplifiers, we studied squeezing as a function of external flux and pump power to explore operating points where Kerr nonlinearity is theoretically minimized. We find that for squeezing operation at a fixed frequency, Kerr varied by about a factor of two and the achievable squeezing showed no significant dependence on Kerr. Rather than Kerr, the squeezing is dominated by internal resonator loss and insertion loss in the microwave chain as confirmed by theoretical modeling. These results indicate that, in practical SPAs, reducing loss, rather than suppressing Kerr, is the primary route to improved squeezing performance.

==> squeezingTheory_new.tex <==
The unitary operator that generates squeezing in a harmonic oscillator with lowering operator $\hat{a}$ is
\begin{equation}\label{eq:squeezingOperator}
    \hat{S}(z) = \exp\!\left[\frac{1}{2}\left(z^*\hat{a}^2 - z\hat{a}^{\dagger 2}\right)\right],
\end{equation}
where $z$ is the squeezing parameter~\cite{gerry_introductory_2008}. 
%In superconducting quantum circuit implementations, to first order, this transformation is exactly that realized by the broad class of degenerate parametric amplifiers (DPA). Phase sensitive and phase preserving gain in a DPA result from application of the squeezing operator to an input field.
In superconducting quantum circuit implementations, this transformation can be realized on traveling microwave fields by a degenerate parametric amplifiers (DPA).

The SNAIL parametric amplifier is a DPA whose nonlinearity can be tuned in situ via magnetic flux applied to the SNAIL, enabling strong three-wave mixing that generates the desired squeezing while simultaneously suppressing unwanted higher‑order nonlinearities.
The SPA Hamiltonian can be written as
\begin{equation}
    \hat{H}/\hbar = \omega_0 \hat{a}^\dagger \hat{a} + g_3(\hat{a}+\hat{a}^\dagger)^3 + g_4(\hat{a}+\hat{a}^\dagger)^4 + \cdots,
\end{equation}
where $\omega_0$ is the resonance frequency and $g_i$ denote the $i$-th order nonlinear coefficients arising from the SNAIL potential~\cite{spa1}. Both $\omega_0$ and $g_i$ depend on device design and are tunable with external flux $\Phi_{\mathrm{ext}}$. Crucially, the fourth-order nonlinearity $g_4$ vanishes near $\Phi_{\mathrm{ext}}\approx0.4\Phi_0$~\cite{snail, spa1}, potentially allowing  parametric amplification and squeezing from an almost ideal three-wave-mixing DPA. However, as shown in Refs.~\cite{spa1,spa2}, higher-order Hamiltonian corrections and pump‑induced effects complicate this condition. 

In practical applications, the squeezing frequency $\omega_s$ is fixed by the downstream system, such as a qubit readout cavity~\cite{eddins_stroboscopic_2018} or the probe frequency in a quantum sensing experiment \cite{bienfait_magnetic_2017, malnou_squeezed_2019, backes_quantum_2021}, . For a three-wave-mixing DPA, the $\omega_s$ is set by the pump frequency $\omega_p$ such that $\omega_s = \omega_p/2$. Assuming the pump is near twice the resonance frequency $\omega_0$, the SPA effective Hamiltonian in a frame rotating at the pump frequency becomes
\begin{equation}
    \hat{H}_{\mathrm{eff}}/\hbar = \Delta_\mathrm{eff} \hat{a}^\dagger \hat{a} + \frac{g_\mathrm{eff}}{2}(\hat{a}^2 + \hat{a}^{\dagger 2}) + \frac{K}{2}\hat{a}^{\dagger 2}\hat{a}^2.
\end{equation}
The parameters $\Delta_\mathrm{eff}$, $g_\mathrm{eff}$ and $K$ depend on all the nonlinearities of $\hat{H}$ as well as the pumping condition. Analytical expressions for these parameters were derived in Refs.~\cite{spa1, spa2}. To lowest order: (1) the effective detuning is $\Delta_\mathrm{eff} = \Delta + \frac{8}{9}K n_p$ where $\Delta = \omega_0 - \omega_p/2$ is the pump-resonator detuning; (2) the squeezing rate is $g_\mathrm{eff} = 4g_3 \sqrt{n_p}$ where $n_p = |\alpha_p|^2$ is the pump-induced intra-resonator photon number, and $\alpha_p$ is the corresponding amplitude; (3) the Kerr nonlinearity $K$, capturing residual four-wave mixing, depends on both $g_3$, $g_4$, and the pump photon number $n_p$, and to lowest order is~\cite{spa2}
\begin{equation}\label{eq:kerr}
    K(n_p) = 12\!\left(g_4 - 5\frac{g_3^2}{\omega_a}\right) + O(n_p) = 12g_4^* + O(n_p).
\end{equation}
%Consequently, tuning $\Delta$ corresponds to tuning $\omega_a$ using the external flux $\Phi_{\mathrm{ext}}$. 
In practice, however, directly predicting $K(n_p)$ from perturbation theory is unreliable; instead, we adopt an experimentally motivated approach and estimate $|K(n_p)|$ using intermodulation‑distortion (IMD) measurements.

The second term of $\hat{H}_\mathrm{eff}$ generates the squeezing interaction whose dynamics correspond to the unitary in Eq.~\ref{eq:squeezingOperator}. Its strength is set in situ by the pump power $P_p\propto n_p$. The effective detuning $\Delta_\mathrm{eff}$ is straightforward to set to zero experimentally, even for fixed $\omega_p/2$, by adjusting $\Phi_{\mathrm{ext}}$ to change $\omega_0$ and thus $\Delta$. By contrast, the Kerr term $K$ is parasitic and cannot be tuned independent of the other two terms of $\hat{H}_\mathrm{eff}$, raising the question of whether its effects can be minimized in practice to realize the squeezing unitary with high fidelity.


%ext consider the gain and squeezing obtained
To understand how $\hat{H}_\mathrm{eff}$ affects traveling fields incident on the SPA, we use the quantum Langevin equation and input–output theory. The SPA resonator is assumed to be coupled to a transmission line with external coupling rate $\kappa_\mathrm{ext}$. Neglecting internal loss for the moment, the total loss rate $\kappa = \kappa_\mathrm{ext}$. In this situation, the phase-preserving power gain is obtained via semi-classical harmonic balance analysis, previously described in Refs.~\cite{spa1,spa2} and generalized in Appendix~\ref{app:spa-squeezing}. The reflection gain for an incident signal at frequency $\omega_p/2$ is 
\begin{equation}
    G_{\mathrm{IL}} = 1 + \frac{\kappa^2g_\mathrm{eff}^2}{\left(\Delta_\mathrm{eff}^2+(\kappa/2)^2-g_\mathrm{eff}^2\right)}.\label{eq:gain}
\end{equation}
Here $G_{\mathrm{IL}}$ is the power gain in reflection referenced to unity transmission, which differs from the common experimental definition where the gain is referenced to the transmission with the SPA pump turned off. As discussed in Appendix~\ref{app:spa-squeezing}, this distinction becomes important in the presence of loss. At $\omega_p/2$, amplification is phase-sensitive, with the phase of the amplified quadrature $\theta$ set by the phase of the pump drive. The amplitude gain of the amplified quadrature is $\sqrt{G_{\mathrm{IL}}}+\sqrt{G_{\mathrm{IL}}-1}$, while the amplitude gain of the squeezed quadrature is $\sqrt{G_{\mathrm{IL}}}-\sqrt{G_{\mathrm{IL}}-1}$.

From Eq.~\ref{eq:gain}, the gain increases with $n_p$ as $g_\mathrm{eff}$ approaches the parametric instability threshold $\sqrt{\Delta_\mathrm{eff}^2+(\kappa/2)^2}$.  The corresponding vacuum squeezing, with no input, is calculated in Appendix~\ref{app:spa-squeezing}. In the ideal, lossless limit, the squeezed-quadrature variance of the output field is
\begin{equation}
    \mathcal{S}_{\text{min}}
    = \frac{1}{2}
      \left(\sqrt{G_{\mathrm{IL}}} - \sqrt{G_{\mathrm{IL}}-1}\right)^{2}.\label{eq:SminGain}
\end{equation}
Thus, $\mathcal{S}_{\text{min}}$ is not independently tunable from $G_{\mathrm{IL}}$. Instead amplification and squeezing from a parametric amplifier are inextricably linked, and $\mathcal{S}_{\text{min}}$ decreases monotonically to zero as $G_{\mathrm{IL}}\rightarrow\infty$.

Within this linearized description, the explicit role of $K$ is to induce a pump‑dependent Stark shift, causing $\Delta_{\mathrm{eff}}\neq\Delta$ and limiting the maximum achievable gain for fixed $\Delta$ and thus the minimum $\mathcal{S}_{\text{min}}$.  However, if pump parameters ($\Delta$, $n_p$) are adjusted to reach the desired gain, then the squeezed‑quadrature variance is insensitive to $K$ to leading order.

In practice, losses and added noise are always present and arise from two sources: (1) internal dissipation of the SPA resonator, modeled by an internal loss rate $\kappa_\mathrm{int}$ giving $\kappa=\kappa_\mathrm{ext}+\kappa_\mathrm{int}$; and (2) attenuation and added noise of the measurement chain, modeled by an efficiency $\eta < 1$. As shown in Appendix~\ref{app:spa-squeezing}, internal loss destroys the one‑to‑one relation between squeezing and gain given by Eq.~\ref{eq:SminGain}. Nevertheless, when $\Delta_\mathrm{eff}=0$, the observed squeezing obeys
\begin{align}
    \mathcal S_{\mathrm{obs}}=\frac{1}{2}-\frac{(\eta\kappa_{\mathrm{ext}})\,g_{\text{eff}}}{(g_{\text{eff}}+\kappa/2)^2}.
\end{align}
The full expression for general $\Delta_\mathrm{eff}$ is given in Appendix~\ref{app:spa-squeezing}, Eq.~\ref{eq:Sobs}. Importantly, for $\Delta_\mathrm{eff}=0$, $\mathcal S_{\mathrm{obs}}$ is independent of $K$. Although this conclusion initially seems at odds with earlier theoretical work~\cite{boutin_effect_2017}, the discrepancy is explained by the fact that contemporary SPAs exhibit extremely small values of $K/\kappa$. Figure~\ref{fig:projections} in Appendix~\ref{app:spa-squeezing} shows numerically calculated gain and squeezing for realistic parameters of state‑of‑the‑art SPAs, confirming that $\mathcal S_{\mathrm{obs}}$ depends negligibly on $K$ provided that $\Delta_\mathrm{eff}$ can be tuned to zero by adjusting $n_p$ and $\Delta$.

In the following sections, we experimentally investigate how $\mathcal S_{\mathrm{obs}}$ depends on $n_p$ and $\Delta$, under the practical constraint that the squeezing frequency is fixed at $\omega_s=\omega_p/2$.

%In practical experiments, the squeezing frequency $f_s$ is fixed by the downstream system, such as the readout cavity of a qubit~\cite{eddins_stroboscopic_2018}. Consequently, $\Delta$ and $\Phi_{\mathrm{ext}}$ cannot both be freely tuned. Unlike typical SPA operation as an output amplifier, where a gain $G = |S_{21,\mathrm{on}}|/|S_{21,\mathrm{off}}|$ of 20~dB is standard, there is no typical gain target for squeezing~\cite{qiu_broadband_2023}. This flexibility allows adjustment of pump power, which modifies $K$ through its dependence on intracavity photon number $n_p$. Combined with detuning introduced by varying $\Phi_{\mathrm{ext}}$, this provides a pathway to identify operating points with reduced $|K|$ and improved squeezing.

==> squeezingTheory_original.tex <==
Quantum squeezing in the microwave domain is commonly implemented using superconducting parametric amplifiers~\cite{castellanos-beltran_amplification_2008, lvovsky_continuous-variable_2009, eichler_observation_2011, perelshtein_broadband_2022, qiu_broadband_2023, vaartjes_strong_2023, mallet_quantum_2011, malnou_optimal_2018, boutin_effect_2017}. The unitary operator that generates squeezing is
\begin{equation}\label{eq:squeezingOperator}
    \hat{S}(z) = \exp\!\left[\frac{1}{2}\left(z^*\hat{a}^2 - z\hat{a}^{\dagger 2}\right)\right],
\end{equation}
where $z$ is the squeezing parameter and $\hat{a}$ the annihilation operator~\cite{gerry_introductory_2008}. 

An ideal three-wave mixing degenerate parametric amplifier (DPA) with resonant mode $\hat{a}$ has Hamiltonian 
\begin{equation}
    \hat{H}/\hbar = \omega_a \hat{a}^\dagger \hat{a} + g_3(\hat{a}+\hat{a}^\dagger)^3+\xi_p(a e^{-i\omega_p t}+a^\dagger e^{i\omega_p t}),
\end{equation}
where $\xi_p$, $\omega_p$ is the pump amplitude and frequency. Assuming $\omega_p = 2\omega_a$,
the interaction Hamiltonian under the rotating-wave approximation becomes
\begin{equation}
    \hat{H}_{\mathrm{int}}/\hbar =  g_3\xi_p\left(\hat{a}^2 + \hat{a}^{\dagger 2}\right),
\end{equation}
and the time-evolution operator $U = e^{-i\hat{H}_{\mathrm{int}}t/\hbar}$ takes the form of the squeezing operator in Eqn.~\ref{eq:squeezingOperator}, with $z = g_3\xi_pt$.

Parametric amplification and squeezing are therefore intrinsically linked: an amplifier operated in phase-sensitive mode applies the squeezing operation to the input state. A larger $|z|$ corresponds to higher gain $G$. Thus, a squeezed vacuum state at frequency $f_s$ can be generated in a three-wave mixing amplifier pumped at $2f_s$, provided the input is the vacuum.

The SPA is a three-wave mixing amplifier, whose Hamiltonian can be written as
\begin{equation}
    \hat{H}/\hbar = \omega_a \hat{a}^\dagger \hat{a} + g_3(\hat{a}+\hat{a}^\dagger)^3 + g_4(\hat{a}+\hat{a}^\dagger)^4 + \cdots,
\end{equation}
where $g_i$ depend on device design and are insitu-tunable with external flux $\Phi_{\mathrm{ext}}$ applied to the SNAIL loops. Crucially, the fourth-order nonlinearity $g_4$ vanishes at $\Phi_{\mathrm{ext}}\approx0.4\Phi_0$~\cite{snail, spa1}, potentially allowing for parametric amplification and squeezing from a near-ideal three-wave-mixing DPA. Higher-order Hamiltonian terms corrections and the presence of the three-wave-mixing pump complicate this condition. In the presence of the pump at $\omega_p$ near $2\omega_a$, the SPA effective Hamiltonian becomes
\begin{equation}
    \hat{H}_{\mathrm{eff}}/\hbar = -\Delta \hat{a}^\dagger \hat{a} + g_3\xi_p(\hat{a}^2 + \hat{a}^{\dagger 2}) + \frac{K}{2}\hat{a}^{\dagger 2}\hat{a}^2, 
\end{equation}
where $\Delta = \omega_a - \omega_p/2$, and the Kerr-nonlinearity $K$ captures the effect of parasitic four-wave mixing up to lowest order. Including terms up to $g_6$ in a harmonic-balance analysis shows that $K$ depends not only on $g_4$ but also on number of pump photons $n_p=|\xi_p|^2$~\cite{spa2} as
\begin{equation}\label{eq:kerr}
    K(n_p) = 12\!\left(g_4 - 5\frac{g_3^2}{\omega_a}\right) + O(n_p) = 12g_4^* + O(n_p).
\end{equation}
An operating point can still be found where $|K|$ is significantly reduced by adjusting the detuning $\Delta$ and external flux $\Phi_{\mathrm{ext}}$. This reduction has been observed to lessen intermodulation distortion and improve power handling compared to the standard $\Delta = 0$ operating point~\cite{spa2}. Here, we investigate whether this property also enhances squeezing performance, as predicted by theory~\cite{boutin_effect_2017}.

In practical experiments, the squeezing frequency $f_s$ is fixed by the downstream system, such as the readout cavity of a qubit~\cite{eddins_stroboscopic_2018}. Consequently, $\Delta$ and $\Phi_{\mathrm{ext}}$ cannot both be freely tuned. Unlike typical SPA operation as an output amplifier, where a gain $G = |S_{21,\mathrm{on}}|/|S_{21,\mathrm{off}}|$ of 20~dB is standard, there is no typical gain target for squeezing~\cite{qiu_broadband_2023}. This flexibility allows adjustment of pump power, which modifies $K$ through its dependence on intracavity photon number $n_p$. Combined with detuning introduced by varying $\Phi_{\mathrm{ext}}$, this provides a pathway to identify operating points with reduced $|K|$ and improved squeezing.



%Because $z$ is linked to amplifier gain, and gain depends on $n_p$, finding an operating point with large $|z|$ and minimal $|K|$ is nontrivial. Fixing $f_s$ for compatibility with a downstream device adds an additional constraint. To address this, a detuning $\Delta = \omega_a - \omega_p/2$ is introduced by varying $\Phi_{\mathrm{ext}}$, where $\omega_p$ is the pump frequency. This approach decouples $n_p$ from $G$, enabling a search for operating points with high gain, minimal Kerr, and optimal squeezing at a specified $f_s$~\cite{spa2}.

